BLIAM: Literature-based Data Synthesis for Synergistic Drug Combination Prediction

Language models pre-trained on scientific literature corpora have substantially advanced scientific discovery by offering high-quality feature representations for downstream applications. However, these features are often not interpretable, and thus can reveal limited insights to domain experts. Instead of obtaining features from language models, we propose BLIAM, a literature-based data synthesis approach to directly generate training data points that are interpretable and model-agnostic to downstream applications. The key idea of BLIAM is to create prompts using existing training data and then use these prompts to synthesize new data points. BLIAM performs these two steps iteratively as new data points will define more informative prompts and new prompts will in turn synthesize more accurate data points. Notably, literature-based data augmentation might introduce data leakage since labels of test data points in downstream applications might have already been mentioned in the language model corpus. To prevent such leakage, we introduce GDSC-combo, a large-scale drug combination discovery dataset that was published after the biomedical language model was trained. We found that BLIAM substantially outperforms a non-augmented approach and manual prompting in this rigorous data split setting. BLIAM can be further used to synthesize data points for novel drugs and cell lines that were not even measured in biomedical experiments. In addition to the promising prediction performance, the data points synthesized by BLIAM are interpretable and model-agnostic, enabling in silico augmentation for in vitro experiments.

==> figures-latex/figure_full_data.tex <==
\begin{figure*}[!ht]
  \centering
    \includegraphics[width=0.99\textwidth]{figures/figure_7/metrics.pdf}
  \caption{Performance on the full dataset. Vertical bars represent standard error bars.}
  \label{fig:full-data}
\end{figure*}

==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:con}


\section{Limitation}
\label{sec:limit}

==> sections/figures-placeholder.tex <==

% This file is used as a placeholder to show the figures.
% Everything here is a draft.


\section{Figures (Placeholder)}
\label{sec:figure}


\begin{figure*}[!ht]
  \centering
    \includegraphics[width=0.99\textwidth]{figures/figure_1/augmentation-white-background.pdf}
  \caption{Overall algorithm process. }
  \label{fig:process}
\end{figure*}



\begin{figure*}
  \centering
    \includegraphics[width=0.99\textwidth]{figures/figure_2/entities.pdf}
  \caption{ Percentage of entities and their appearing sentences/abstracts. (a) The number of sentences containing single drugs, single cell lines, and drug pairs. (b) The number of sentences containing triplets. (c) The number of abstracts containing single drugs, single cell lines, and drug pairs. (d) The number of abstracts containing triplets. }
\end{figure*}


% one figure with four subfigures
\begin{figure*}[!ht]
  \centering
    \includegraphics[width=0.99\textwidth]{figures/figure_3/metrics.pdf}
  \caption{Performance on main experiments evaluated using the four metrics. Vertical bars represent standard error bars.}
  \label{fig:overall_performance}
\end{figure*}

\begin{figure*}[!ht]
  \centering
    \includegraphics[width=0.32\textwidth]{figures/figure_4_5/TSNE Visualization_iter_1.pdf}
    \includegraphics[width=0.32\textwidth]{figures/figure_4_5/TSNE Visualization_iter_2.pdf}
    \includegraphics[width=0.32\textwidth]{figures/figure_4_5/TSNE Visualization_iter_3.pdf}
  \caption{TSNE visualization on sentence embeddings in iteration 1, 2 and 3.}
  \label{fig:tsne}
\end{figure*}



% \begin{figure*}[!ht]
%   \centering
%   \includegraphics[width=0.32\textwidth]{figures/figure_4_5/TSNE Visualization_iter_1.pdf}
%   \caption{Prompt template. Same as figure 4, left here to match the figure numbers in paper structure.}
%   \label{fig:process}
% \end{figure*}



\begin{figure*}[!ht]
  \centering
    \includegraphics[width=0.99\textwidth]{figures/figure_6/metrics.pdf}
  \caption{Performance on unseen combination scenario evaluated using the four metrics. Vertical bars represent standard error bars.}
  \label{fig:unseen_performance}
\end{figure*}



\begin{figure*}[!ht]
  \centering
    \includegraphics[width=0.99\textwidth]{figures/figure_7/metrics.pdf}
  \caption{Performance on the full dataset. Vertical bars represent standard error bars.}
  \label{fig:full-data}
\end{figure*}
